High-Throughput SAT Sampling

In this work, we present a novel technique for GPU-accelerated Boolean satisfiability (SAT) sampling. Unlike conventional sampling algorithms that directly operate on conjunctive normal form (CNF), our method transforms the logical constraints of SAT problems by factoring their CNF representations into simplified multi-level, multi-output Boolean functions. It then leverages gradient-based optimization to guide the search for a diverse set of valid solutions. Our method operates directly on the circuit structure of refactored SAT instances, reinterpreting the SAT problem as a supervised multi-output regression task. This differentiable technique enables independent bit-wise operations on each tensor element, allowing parallel execution of learning processes. As a result, we achieve GPU-accelerated sampling with significant runtime improvements ranging from $33.6\times$ to $523.6\times$ over state-of-the-art heuristic samplers. We demonstrate the superior performance of our sampling method through an extensive evaluation on $60$ instances from a public domain benchmark suite utilized in previous studies.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> table3.tex <==
\scalebox{0.95}{\begin{tabular}{c|c|c|c|c|c||c|c|c|c|c|c} 
\hline
\midrule
CircuitSAT & \# Inputs & \# Outputs & \# Logic Gates & \# DFF & {\sc Demotic} & CircuitSAT & \# Inputs & \# Outputs & \# Logic Gates & \# DFF & {\sc Demotic}\\ 
 \midrule
s$27$    & $4$   & $1$   & $10$   & $3$  & $\mathbf{110,014}$ & s$1196$ & $14$ & $14$ & $529$ & $18$ & $\mathbf{355}$\\
s$208.1$ & $10$  & $1$   & $104$  & $8$   & $\mathbf{135,950}$ & s$1238$ & $14$ & $14$ & $508$ & $18$ & $\mathbf{18,718}$\\  
s$298$   & $3$   & $6$   & $119$  & $14$  & $\mathbf{28,947}$ & s$1269$ & $14$ & $10$ & $569$ & $37$ & $\mathbf{4,827}$\\  
s$344$   & $9$   & $11$  & $160$  & $15$  & $\mathbf{50,124}$ & s$1423$ & $17$ & $5$ & $657$ & $74$ & $\mathbf{6,860}$\\ 
s$349$   & $9$   & $11$  & $161$  & $15$  & $\mathbf{77,532}$ & s$1488$ & $8$ & $19$ & $653$ & $6$ & $\mathbf{4,534}$\\ 
s$382$   & $3$   & $6$   & $158$  & $21$  & $\mathbf{88,286}$ & s$1494$ & $8$ & $19$ & $647$ & $6$ & $\mathbf{2,949}$\\ 
s$386$   & $7$   & $7$   & $159$  & $6$  & $\mathbf{77,136}$ & s$1512$ & $29$ & $21$ & $780$ & $57$ & $\mathbf{3,747}$\\ 
s$400$   & $3$   & $6$   & $164$  & $21$  & $\mathbf{73,807}$ & s$3271$ & $26$ & $14$ & $1572$ & $116$ & $\mathbf{719}$\\ 
s$420.1$ & $18$  & $1$   & $118$  & $16$  & $\mathbf{69,216}$ & s$3330$ & $40$ & $73$ & $1789$ & $132$ & $\mathbf{56}$\\ 
s$444$   & $3$   & $6$   & $181$  & $21$  & $\mathbf{72,897}$ & s$3384$ & $43$ & $26$ & $1685$ & $183$ & $\mathbf{933}$\\ 
s$499$   & $1$   & $22$  & $152$  & $22$  & $\mathbf{50,983}$ & s$4863$ & $49$ & $16$ & $2342$ & $104$ & $\mathbf{565}$\\ 
s$510$   & $19$  & $7$   & $211$  & $6$  & $\mathbf{25,519}$ & s$5378$ & $35$ & $49$ & $2779$ & $179$ & $\mathbf{525}$\\ 
s$526$   & $3$   & $6$   & $193$  & $21$  & $\mathbf{53,251}$ & s$6669$ & $83$ & $55$ & $3080$ & $239$ & $\mathbf{107}$\\ 
s$526n$  & $3$   & $6$   & $194$  & $21$  & $\mathbf{57,926}$ & s$9234.1$ & $36$ & $39$ & $5597$ & $211$ & $\mathbf{20}$\\ 
s$635$   & $2$   & $1$   & $286$  & $128$  & $\mathbf{44,236}$ & s$9234$ & $19$ & $22$ & $5597$ & $228$ & $\mathbf{547}$\\ 
s$641$   & $35$ & $24$ & $379$ & $19$  & $\mathbf{37,267}$ & s$13207.1$ & $62$ & $152$ & $7951$ & $638$ & $\mathbf{334}$\\ 
s$713$   & $35$ & $23$ & $393$ & $19$  & $\mathbf{35,937}$ & s$13207$ & $31$ & $121$ & $7951$ & $669$ & $\mathbf{310}$\\ 
s$820$   & $18$ & $19$ & $289$ & $5$  & $\mathbf{22,229}$ & s$15850.1$ & $77$ & $150$ & $9772$ & $534$ & $\mathbf{100}$\\ 
s$832$   & $18$ & $19$ & $287$ & $5$  & $\mathbf{21,373}$ & s$15850$ & $14$ & $87$ & $9772$ & $597$ & $\mathbf{101}$\\ 
s$838.1$ & $34$ & $1$  & $446$ & $32$  & $\mathbf{30,482}$ & s$35932$ & $35$ & $320$ & $16065$ & $1728$ & $\mathbf{13}$\\ 
s$938$   & $34$ & $1$ & $446$ & $32$  & $\mathbf{27,234}$ & s$38417$ & $28$ & $106$ & $22179$ & $1636$ & $\mathbf {15}$\\ 
s$953$   & $16$ & $23$ & $395$ & $29$  & $\mathbf{4,964}$ & s$38584.1$ & $38$ & $304$ & $19253$ & $1426$ &  $\mathbf {2}$\\ 
s$967$   & $16$ & $23$ & $394$ & $29$  & $\mathbf{30,228}$ & s$38584$ & $12$ & $278$ & $19253$ & $1452$ & $\mathbf {2}$ \\ 
s$991$   & $65$ & $17$ & $519$ & $19$ & $\mathbf{6,932}$ &  \\
\midrule
\hline
\end{tabular}}
